6D Camera Relocalization in Visually Ambiguous Extreme Environments

We propose a novel method to reliably estimate the pose of a camera given a sequence of images acquired in extreme environments such as deep seas or extraterrestrial terrains. Data acquired under these challenging conditions are corrupted by textureless surfaces, image degradation, and presence of repetitive and highly ambiguous structures. When naively deployed, the state-of-the-art methods can fail in those scenarios as confirmed by our empirical analysis. In this paper, we attempt to make camera relocalization work in these extreme situations. To this end, we propose: (i) a hierarchical localization system, where we leverage temporal information and (ii) a novel environment-aware image enhancement method to boost the robustness and accuracy. Our extensive experimental results demonstrate superior performance in favor of our method under two extreme settings: localizing an autonomous underwater vehicle and localizing a planetary rover in a Mars-like desert. In addition, our method achieves comparable performance with state-of-the-art methods on the indoor benchmark (7-Scenes dataset) using only 20% training data.

==> figures/7scenes.tex <==
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.75\linewidth]{imgs/7scenes.png}
    \caption{Camera trajectory results and SfM reconstruction on 7-Scenes dataset. }
    \label{fig:7scenes}
 \end{figure}

==> figures/train_test.tex <==
\begin{figure}[t!]
    \centering
    \subfigure[Harbor site 2]{\includegraphics[width=0.4\linewidth]{imgs/train_aq.jpg}}
    \subfigure[G1 location]{\includegraphics[width=0.4\linewidth]{imgs/train_mars.jpg}}
    \vspace{-10pt}
    \caption{Experimental setup: train and test splits of sequences from (a) Aqualoc~\cite{ferrera2019aqualoc} and (b) Mars-analog dataset~\cite{meyer2021madmax}.}
    \label{fig:train_test_split}
\end{figure}
